Sound Concurrent Traces for Online Monitoring Technical Report

Monitoring concurrent programs typically rely on collecting traces to abstract program executions. However, existing approaches targeting general behavioral properties are either not tailored for online monitoring, are no longer maintained, or implement naive instrumentation that often leads to unsound verdicts. We first define the notion of when a trace is representative of a concurrent execution. We then present a non-blocking vector clock algorithm to collect sound concurrent traces on the fly reflecting the partial order between events. Moreover, concurrent events in the representative trace pose a soundness problem for monitors synthesized from total order formalisms. For this, we extract a causal dependence relation from the monitor to check if the trace has the needed orderings and define the conditions to decide at runtime when a collected trace is monitorable. We implement our contributions in a tool, FACTS, which instruments programs compiling to Java bytecode, constructs sound representative traces, and warns the monitor about non-monitorable traces. We evaluate our work and compare it with existing approaches.

==> Makefile <==
all: build

FLAGS=--shell-escape --synctex=1

quick:
	pdflatex ${FLAGS} main
build:
	pdflatex ${FLAGS} main
	bibtex main
	pdflatex ${FLAGS} main
	pdflatex ${FLAGS} main

check:
	cat main.log | grep -E -n '\(\..*\.tex\ |Overfull'

clean:
	@rm *.cut *.out *.log *.aux *.fls *.fdb_latexmk _*.* *.mtc* *.synctex.gz *.maf *.blg *.bbl *.toc *.thm _minted-* 2>/dev/null || true
	@rm -rf _minted-* 2>/dev/null || true


==> figures.tex <==
\section{Figures}
\begin{figure}[H]
    \centering
    \scalebox{0.85}{\input{tikz/rw-full-aligned.tex}}
    \caption{%
    rw-full-aligned
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H]
    \centering
    \scalebox{0.85}{\input{tikz/rw-full.tex}}
    \caption{%
    rw-full
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H]
    \centering
    \scalebox{0.85}{\input{tikz/rw-full-regions.tex}}
    \caption{%
    rw-full-regions
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H] 
    \centering
    \scalebox{0.85}{\input{tikz/rw.tex}}
    \caption{%
       rw
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H]
    \centering
    \scalebox{0.85}{\input{tikz/rw-project.tex}}
    \caption{%
        rw-project
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H]
    \centering
    \scalebox{0.85}{\input{tikz/rw-channel.tex}}
    \caption{%
        rw-channel
    }
    \label{fig:rw-full}
\end{figure}


\begin{figure}[H] 
    \centering
    \scalebox{0.85}{\input{tikz/rw-sync.tex}}
    \caption{%
       rw-sync
    }
    \label{fig:rw-full}
\end{figure}

\begin{figure}[H] 
    \centering
    \scalebox{0.85}{\input{tikz/rw-actions.tex}}
    \caption{%
       rw-actions
    }
    \label{fig:rw-full}
\end{figure}

 
\begin{figure}[H] 
    \centering
    \scalebox{0.85}{\input{tikz/params.tex}}
    \caption{%
       params
    }
    \label{fig:rw-channel}
\end{figure}
\begin{figure}[H] 
    \centering
    \scalebox{0.85}{\input{tikz/overview0.tex}}
    \caption{%
    overview
    }
    \label{fig:rw-channel}
\end{figure}

\begin{figure}[H] 
    \centering
    \scalebox{1}{\input{tikz/no-rw-between-w.tex}}
    \caption{%
    overview
    }
    \label{fig:rw-channel}
\end{figure}

==> newtheorems.tex <==
\theoremstyle{plain}
\theorembodyfont{\upshape}
% \theoremsymbol{\ensuremath{\ast}}
\theoremseparator{}
\newtheorem{Exemple}{Exemple}

\theoremstyle{break}
\theoremheaderfont{\sc}
\theorembodyfont{\upshape}
\theoremstyle{nonumberplain}
\theoremseparator{~:}
\theoremsymbol{\rule{1ex}{1ex}}
\theorempostwork{\qed}
\newtheorem{Preuve}{Preuve}

\theoremstyle{plain}
\theorembodyfont{\upshape}
\theoremsymbol{\ensuremath{\ast}}
\theoremseparator{}
\newtheorem{Remarque}{Remarque}


\theoremstyle{plain}
\theoremseparator{.}
\theoremprework{\bigskip\hrule}
\theorempostwork{\hrule\bigskip}
\theoremsymbol{}
\newtheorem{Definition}{Definition}


\theoremstyle{plain}
\theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
\theoremsymbol{\ensuremath{\diamondsuit}}
\theoremseparator{~:}
\newtheorem{Propriete}{Propriete}


\theoremstyle{plain}
\theoremsymbol{\ensuremath{\diamondsuit}}
\theoremindent0.5cm
\theoremnumbering{greek}
\newtheorem{Lemme}{Lemme}

\theoremstyle{plain}
\theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
\theoremsymbol{}
\theoremseparator{~:}
\newtheorem{Theorem}{Theorem}




% \theoremclass{Theorem}
% \theoremstyle{plain}
% \newshadedtheorem{ImportantTheorem}[Theorem]{Theorem}
% 
% 
% 
% \theoremclass{Theorem}
% \theoremstyle{break}
% \shadecolor{red}
% \newshadedtheorem{vImportantTheorem}{Theorem}{Theorem}
% 
% 
% 
% 

\theoremstyle{plain}
\theoremheaderfont{\normalfont\bfseries}\theorembodyfont{\slshape}
\theoremsymbol{\ensuremath{\diamondsuit}}
\theoremseparator{:}
\newtheorem{Corollaire}{Corollaire}




 

==> notation-TN.tex <==
\newcommand\mb[1]{\ensuremath{\boldsymbol{#1}}}
\newcommand\mtt[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\sym}{\mathrm}
% \newcommand\equiva{\Leftrightarrow}
\newcommand{\matchr}{{\kern 0 em \rightarrow\,}}
\newcommand{\matchc}{|\>}
\newcommand\THEMIS{\texttt{THEMIS}}
\newcommand{\vars}{\texttt}
\newcommand{\func}{\mathrm}
\newcommand{\funca}{\textsc}
\newcommand{\code}[1]{\ensuremath{\mathtt{#1}}}
\newcommand{\cls}[1]{\textsc{#1}}
\newcommand{\ltlk}[1][3]{\mathrm{LTL}_{#1}}
%\newcommand{\meth}[1]{\texttt{#1}}
\newcommand{\meth}[2][blue]{%
\if\instring{(}{#2}%
\mintinline{java}{#2}%
\else%
\texttt{\footnotesize{{\color{#1}#2}}}%
\fi
}
\newcommand{\bashcmd}[1]{\mintinline{bash}{#1}}
\newcommand\xv{x}
\DeclareMathOperator{\fdom}{dom}
\DeclareMathOperator{\fcodom}{codom}
\newcommand\pif[1][\>]{\ensuremath{#1 \mbox{\text{if }}}}
\newcommand\pelse[1][\>]{\ensuremath{#1 \mbox{\text{otherwise}}}}
\newcommand\tuple[1]{\langle #1 \rangle}
\newcommand\aut{\mathcal{A}}
\newcommand\event{\mathcal{E}}
\newcommand\mem{\mathcal{M}}
\newcommand\Mem{\mathit{Mem}}
\newcommand\sys{\mathcal{I}}
\newcommand\rec{\mathcal{R}}
\newcommand\net{\mathcal{N}}
\newcommand\verdict{\mathbb{B}_3}
\newcommand\verdictb{\mathbb{B}_2}
\newcommand\booldomain{\mathbb{B}}
\newcommand\timestamp{\mathbb{N}}
\newcommand\trange{\mathcal{R}}
\newcommand\jump{\vspace{1cm}}
%\newcommand\sysadd{\uplus}
\newcommand\sysadd{\dagger_{\lor}}
\newcommand\memadd{\dagger_2}
\newcommand\sMem{\mathit{Mem}}
\newcommand\atoms{\mathit{Atoms}}
\newcommand\chorcoref{\mathit{coref}}
\newcommand\chorref{\mathit{ref}}
\newcommand\chorresp{\mathit{respawn}}
\newcommand\scor{\mathrm{scor}}
\newcommand\chorkill{\mathit{kill}}
\newcommand\msgkill{\mathrm{msg}_{\rm kill}}
\newcommand\msgverdict{\mathrm{msg}_{\rm ver}}
\newcommand\expr{\mathit{Expr}}
\newcommand\clookup{\mathrm{lu}}
\newcommand\cchoose{\mathrm{chc}}
\newcommand\csplit{\mathrm{split}}
\newcommand\verdictf{\mathrm{ver}}
\newcommand\verdictAt{\mathrm{verAt}}
\newcommand\seval{\func{eval}}
\newcommand\senc{\func{enc}}
\newcommand\sstore{\mathrm{store}}
\newcommand\AP{\mathit{AP}}
\newcommand\APmons{{\mathit{AP}_{\mathrm{mons}}}}
\newcommand\smove{\mathrm{mov}}
\newcommand\sreach{\mathrm{sel}}
\newcommand\sto{\mathrm{to}}
\newcommand\snext{\mathrm{next}}
\newcommand\Net{\mathrm{gnet}}
\newcommand\MONID{\mathrm{m}}
\newcommand\paths{\ensuremath{\mathrm{paths}}}
\newcommand\mondep{\mathrm{dep}}
\newcommand\mons{\mathrm{Mons}}
\newcommand\comps{\mathcal{C}}
\newcommand\decspec{\mathit{A_\mathrm{D}}}
\newcommand\setof[1]{\{#1\}}
\newcommand\trace{\mathrm{tr}}
\newcommand\vna{\mathtt{\mathbf{?}}}
\newcommand\vt{\ensuremath{\mathtt{true}}}
\renewcommand\vt{\ensuremath{\top}}
\newcommand\vf{\ensuremath{\mathtt{false}}}
\renewcommand\vf{\ensuremath{\bot}}
\newcommand\fundef{\mathrm{undef}}
\newcommand\cons{\mathrm{memc}}
\newcommand\migrchc{\mathrm{choose}}
\newcommand\sresolve{\mathrm{res}}
\newcommand\rw{\mathrm{rw}}
\newcommand\fid{\mathrm{idt}}
\newcommand\fts{\mathrm{ts}}
\newcommand\fsimp{\mathrm{simplify}}
\newcommand\finc{\mathrm{inc}}
\newcommand\moveq{\func{moveq}}
\newcommand\fenc[1]{\ensuremath{\func{s}_{#1}}}
\newcommand\monitorable{\mathrm{monitorable}}
\newcommand\compat{\mathrm{compat}}
\newcommand\constraint{\mathrm{cdep}}
\newcommand\reach[1]{\mathrm{reach}_{\mathrm{#1}}}
% \renewcommand{\algorithmicforall}{\textbf{for each}}

\newcommand\MDG{\ensuremath{\mathrm{MDG}}}
\newcommand\MDS{\ensuremath{\mathrm{MDS}}}

\newcommand\decent{\ensuremath{\mathcal{D}}}
\newcommand\traces{\ensuremath{\mathcal{T}}}
\newcommand\cmapping{\ensuremath{\mathcal{L}}}
\newcommand\mroot{\ensuremath{\mathrm{rt}}}
\newcommand\emptytrace{\ensuremath{\epsilon}}

\newcommand\LTLT{\ensuremath{\mathrm{LTL_3}}}
\newcommand\paramlabel{L}
\newcommand\paramoedge{P}
\newcommand\paramdelay{\delta_{t}}%
\def\MemRep{\texttt{EHE}}
\newcommand\sstable{\mathrm{kn}}
\newcommand\algorch{Orch}
\newcommand\algmigr{Migr}
\newcommand\algmigrr{Migrr}
\newcommand\algchor{Chor}
\newcommand{\sproject}{\upharpoonleft}
\newcommand{\timestamps}[1]{\ensuremath{\mathrm{rounds}({#1})}}
\newcommand{\xiff}{\mbox{ if }}
\newcommand{\xelse}{\mbox{ otherwise}}
\newcommand{\funcparts}[2][ll]
{
	\left\{
		\begin{array}{#1}
			#2
		\end{array}
	\right.
}
\newcommand{\ifbig}[1] {
  \begin{array}{l}\pif #1\end{array}
}
\newcommand{\ifskip}{\\ \quad \>}
\newcommand{\twopartdef}[3]
{
	\left\{
		\begin{array}{ll}
			#1 & \mbox{if } #2 \\
			#3 & \mbox{otherwise}
		\end{array}
	\right.
}
\newcommand{\mrm}[1]{\mathrm{#1}}


\newcommand{\rooms}{\ensuremath{\mathcal R}}

\newcommand{\ltlx}[0]{\ensuremath{\boldsymbol{\mathrm{X}}}}
\newcommand{\ltlu}[0]{\ensuremath{\, \boldsymbol{\mathrm{U}}\, }}
%\DeclareMathOperator{\ltlg}{\square}
%\DeclareMathOperator{\ltlf}{\Diamond}
\DeclareMathOperator{\ltlg}{\boldsymbol{\mathrm{G}}}
\DeclareMathOperator{\ltlf}{\boldsymbol{\mathrm{F}}}
\newcommand{\ltlfw}[1]{\ensuremath{\ltlf_{\leq #1}}}
\newcommand{\ltlgw}[1]{\ensuremath{\ltlg_{\leq #1}}}
\newcommand{\propd}[1]{\emph{``#1''}}

\newcommand{\defas}[0]{\stackrel{{\scriptscriptstyle\rm def}}{=}}



\newcommand{\mproptypes}{\ensuremath{\mathbb {P}}}
%
\newcommand{\minput}{\ensuremath{\mathbb {I}}}
\newcommand{\moutput}{\ensuremath{\mathbb {O}}}
\newcommand{\mtid}{\ensuremath{\mathrm {TID}}}
\newcommand{\msid}{\ensuremath{\mathrm {SID}}}
% \newcommand{\mactions}{\ensuremath{\mathbb {A}}}
\newcommand{\nactions}{\ensuremath{\mathbb {NA}}}
\newcommand{\mactionssync}{\ensuremath{\mathbb {SA}}}
\newcommand{\oactions}{\ensuremath{\mathbb {OA}}}
\newcommand{\mspawn}{\ensuremath{\mathbb {S}}}
% \newcommand{\mevents}{\ensuremath{\mathbb {E}}}
\newcommand{\mevents}{\ensuremath{\mathcal {E}}}

\newcommand{\mempty}{\ensuremath{\mathcal{E}}}
\newcommand{\mexec}{\ensuremath{\mathcal{C}}}
\newcommand{\mregion}{\ensuremath{\mathcal{R}}}
\newcommand{\mpart}{\ensuremath{\mathrm{na}}}

% \newcommand{\mm}{\ensuremath{\mathit{m}}}

% \newcommand{\mactions}{\ensuremath{\mathcal {U}}}
% \newcommand{\actexec}{\ensuremath{\mathcal {A}}}
% \newcommand{\mtraceactions}{\ensuremath{\Sigma}}
% \newcommand{\mexecs}{\ensuremath{\mathcal {X}}}
% \newcommand{\mmodels}{\ensuremath{\mathcal {M}}}



\newcommand\dltlna{\mathbb{B}_3}
\newcommand\dints{\mathbb{N}}

\newcommand{\mthreads}{\ensuremath{\mathbb {T}}}
\newcommand{\fspawn}{\ensuremath{\mathrm {spawn}}}
\newcommand{\fpool}{\ensuremath{\mathrm {pool}}}
\newcommand{\fev}{\ensuremath{\mathrm {match}}}
\newcommand{\fsync}{\ensuremath{\mathrm {sync}}}
\newcommand{\fidx}{\ensuremath{\mathrm {idx}}}
\newcommand{\fstate}{\ensuremath{\mathrm {state}}}
\newcommand{\fproj}{\ensuremath{\mathrm {proj}}}

\newcommand{\notify}{\ensuremath{\mathrm {notify}}}

% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}

% \newcommand{\orderthread}{\ensuremath{\xrightarrow{t}}}
% \newcommand{\ordersync}{\ensuremath{\xrightarrow{s}}}
% \newcommand{\ordersw}{\ensuremath{\xrightarrow{s}}}
% \newcommand{\orderprog}{\ensuremath{\xrightarrow{prog}}}
% \newcommand{\ordertr}{\ensuremath{\xrightarrow{tr}}}
\newcommand{\orderna}{\ensuremath{\ \orderexec \cap \ (\nactions \times \nactions)}}
% \newcommand{\orderexec}{\ensuremath{\xrightarrow{e}}}
\newcommand{\observeexec}{\ensuremath{\xrightarrow{o}}}


\newcommand{\locator}{selector} 
\newcommand{\locators}{selectors} 
\newcommand{\Locators}{Selectors} 


\newcommand{\Methods}{{\mathit{Methods}}} 
\newcommand{\Blocks}{{\mathit{Blocks}}} 
\newcommand{\Instrs}{{\mathit{Instrs}}} 
\newcommand{\Shadows}{{\mathit{Shadows}}}

\newcommand{\blocks}{{\mathrm{blocks}}} 
\newcommand{\instrs}{{\mathrm{instrs}}} 


% \newcommand{\mra}{\ensuremath{{\mathcal {U}}_\mathrm{r}}}
% \newcommand{\mera}{\ensuremath{{\mathcal {E}}_\mathrm{r}}}
% \newcommand{\msa}{\ensuremath{{\mathcal {U}}_\mathrm{s}}}
% \newcommand{\mesa}{\ensuremath{{\mathcal {E}}_\mathrm{s}}}
% \newcommand{\mres}{\ensuremath{{\mathcal {R}}}}


\newcommand{\intensity}{\ensuremath{\mathcal {I}}}
\newcommand\TOOL{\code{Paratrace}}
\newcommand{\evs}[1]{\ensuremath{\mathtt{#1}}}

\newcommand{\mm}{\ensuremath{\mathit{m}}}
\newcommand{\mma}{\ensuremath{\actexec_{m}}}
\newcommand{\mmo}{\ensuremath{\rightarrow_{\mathrm{m}}}}
\newcommand{\rcor}{\ensuremath{\mathrm{snd}}}
\newcommand{\rfaith}{\ensuremath{\mathrm{faith}}}
\newcommand{\mactions}{\ensuremath{\mathcal {U}}}
\newcommand{\actexec}{\ensuremath{\mathcal {A}}}
\newcommand{\mtraceactions}{\ensuremath{\Sigma}}
\newcommand{\mexecs}{\ensuremath{\mathcal {X}}}
\newcommand{\mmodels}{\ensuremath{\mathcal {M}}}
\newcommand{\mra}{\ensuremath{{\mathcal {U}}_\mathrm{r}}}
\newcommand{\mera}{\ensuremath{{\mathcal {E}}_\mathrm{r}}}
\newcommand{\msa}{\ensuremath{{\mathcal {U}}_\mathrm{s}}}
\newcommand{\mesa}{\ensuremath{{\mathcal {E}}_\mathrm{s}}}
\newcommand{\mres}{\ensuremath{{\mathcal {R}}}}
\newcommand{\orderstrict}{\ensuremath{\xrightarrow{strict}}}
\newcommand{\ordermem}{\ensuremath{\xrightarrow{mem}}}
\newcommand{\orderexec}{\ensuremath{\xrightarrow{e}}}
\newcommand{\orderthread}{\ensuremath{\xrightarrow{t}}}
\newcommand{\ordersync}{\ensuremath{\xrightarrow{s}}}
\newcommand{\ordersw}{\ensuremath{\xrightarrow{sw}}}
\newcommand{\orderprog}{\ensuremath{\xrightarrow{prog}}}
\newcommand{\ordertr}{\ensuremath{\rightarrow_{\mathrm{t}}}}

\newcommand{\mtr}{\ensuremath{\mathit{t}}}

==> old-writeup.tex <==
 



% We use the notation $\code{id.lbl^{thread}_{resource}}$ and omit the \textit{ctx} information when not needed.
 



% \begin{example}[Concurrent fragment for 1-Writer 2-Readers.]  \label{ex:multirv:rw:root}
%     \textcolor{Blue}{
%     \figref{fig:rw-fragment-full} shows a concurrent execution fragment for a simple \emph{1-Writer 2-Readers} program.
%     A thread can write to a shared variable, and two other threads can read from the variable.
%     %
%     The threads can read concurrently, but no thread can write or read while a write is occurring.
%     %
%     The concurrent execution fragment contains all actions performed by all threads, along with the partial order inferred from locks.
%     We have three locks: test for readers ($\sym{t}$), service ($\sym{s}$), and readers counter ($\sym{c}$).
%     Lock $\sym{t}$ checks if any reader is currently reading, this lock gives preference to writers.
%     Lock $\sym{s}$ is used to regulate access to the shared resource, it can be either obtained by readers or one writer.
%     Lock $\sym{c}$ is used to regulate access to the readers counters, it only synchronizes readers.
%     In this concurrent execution, we have three synchronizations on the resource.
%     First, the writer  acquires the resource and writes.
%     Second, the readers acquire the resource and read in parallel.
%     Third, the writer acquires the resource and  writes.
%     Action $\code{1.l_s^1}$ represents the execution of a lock acquire instruction by a thread with threadid $1$ on the shared resource lock ($\code{s}$).
%     }
%     \end{example}

% \subsection{Threads and Events}

% \paragraph{Distinguishing threads.}
% %
% To allow for dynamic number of threads, we define thread types $\mthreads$, to distinguish threads that are relevant to the specification.
% For example, thread types for \emph{readers-writers} are in the set $\mthreads_{rw} \defas \setof{\mathrm{reader}, \mathrm{writer}}$.
% Thread types allows us to express a property over all threads of the same type.
% %
% In order to assign a type to a thread in practice, we define a set of actions $\mspawn \subseteq \mactions$ called ``spawn'' actions.
% For example in \emph{readers-writers}, we can assign the spawn action of a reader (resp. writer) to be the method invocation of $\code{Reader.run}$ ($\code{Writer.run}$).
% Function $\fspawn : \mspawn \rightarrow \mthreads$, assigns a thread type to a spawn action.
% The threads that match a given type are determined based on the spawn action(s) present during the execution.
% We note that a thread is able to have multiple types.
% %
% To reference all threads assigned a given type, we use function $\fpool : \mthreads \rightarrow 2^{\mtid}$.
% %
% That is, given a type $t$, a thread with threadid $tid \in \fpool(t)$ iff $\exists a \in \mactions: \fspawn(a) = t \land a.\mathrm{threadid} = tid$.
% %
% This approaches allows a thread to have multiple types, as it is possible for different properties to operate on different events in the same given thread.








% \paragraph{Events.}
% Thread types are used to determine threads that are relevant for specific properties.
% For example, we are interested in verifying properties that apply to readers only.
% Properties are evaluated by processing a sequence of events.
% We note that actions ($\mactions$) illustrate information about the program execution at runtime.
% Actions need to be converted to events, that will be processed by the specification.
% As such, we define for each thread type $type \in \mthreads$, the alphabet of events: $\mevents_{type}$.
% The set $\mevents_{type}$ contains all the events that can be generated from actions for the particular thread type $type \in \mthreads$.
% The empty event $\mempty$ is a special event that indicates that no events are matched.
% Then, we provide a total function $\fev_{type} : \mactions \rightarrow  \setof{\mempty} \cup \mevents_{type}$.
% The implementation of $\fev$  relies on the specification formalism used, it is capable of generating events based on the action itself, its label, id or context.
% For example, the conversion can utilize runtime context of actions to generate parametric events when needed.
% We illustrate a simple event alphabet containing atomic propositions, and a function $\fev$ that matches using the label of an action in Example~\ref{ex:def:events}.


% \begin{example}[Events.] \label{ex:def:events}
% We identify for \emph{readers-writers} (\rex{ex:multirv:rw:root}) two thread types:  $\mthreads_{rw} \defas \setof{\mathrm{reader}, \mathrm{writer}}$.
% We are interested in the events $\mevents_\mathrm{reader} \defas \setof{\mathrm{read}}$, and $\mevents_\mathrm{writer} \defas \setof{\mathrm{write}}$.
% For a specification at the level of a given thread, we have either a reader or a writer, the event associated with the reader (resp. writer)  is $\mathrm{read}$ (resp. $\mathrm{write}$).

% \[\begin{array}{ll}
%   \fev_\mathrm{reader}(\sym{a}) \defas \funcparts{
%       \mathrm{read}   & \xiff \sym{a.lbl} = \mbox{``r''}, \\
%       \mempty{}       & \xelse
%   } \quad &
%   \fev_\mathrm{writer}(\sym{a}) \defas \funcparts{
%       \mathrm{write}  & \xiff \sym{a.lbl} =  \mbox{``w''}, \\
%       \mempty{}       & \xelse.
%   }
% \end{array}\]
% While we illustrated a simple case that is sufficient to monitor \emph{readers-writers}, we can also consider more complex cases where events are generated using the action context.
% As such, let us consider the new more complex type $\mathrm{reader'}$.
% Consider that read actions operate on an array of size $n$, and their context contain the index read (stored in the key $\mathrm{ind}$), the reader will read all values in the array starting from the index 0 to $n-1$.
% We define for reading the start and end events: $\mevents_\mathrm{reader'} \defas \setof{\mathrm{startread}, \mathrm{endread}}$.
% We associate them with actions as follows:
% \[
% \fev_\mathrm{reader'}(\sym{a}) \defas \funcparts{
%     \mathrm{startread} & \xiff \sym{a.lbl} = \mbox{``r''} \land \sym{a.ctx}(\mathrm{ind}) = 0, \\
%     \mathrm{endread}   & \xiff \sym{a.lbl} = \mbox{``r''} \land \sym{a.ctx}(\mathrm{ind}) = n-1, \\
%     \mempty{}       & \xelse.
% }
% \]
% \end{example}
% \newpage


==> response.tex <==
Thank you for the reviews. Below are our responses to the posed questions. Some answers are combined.

#129A.1 
The presented algorithm differs from standard algorithms as follows: 
- Processing: It can run asynchronously, allowing scenarios where a delay can be tolerated. Most, if not all VC algorithms in the literature block the execution to process the algorithm at each event. Our algorithm receives events and timestamps them without needing the program to wait (block) before (or after) each event.
- Instrumentation: It does not require advice atomicity. Instead, it just requires instrumenting release/acquire action with @before/@after directives.
- Implementation: It treats reads and writes differently to accommodate the lack of advice atomicity. While accesses to locks (for instance) follow the synchronization order, reads and writes do not. When forced atomicity is used, an algorithm is in fact forcing a linearization on reads and writes (via instrumentation) by requiring a thread to acquire a lock before executing a read or write. However, our algorithm avoids forcing such linearization and can still merge clocks when encountering reads.

#129A.2 
For RQ1, our approach avoids interfering with the parallel execution in two ways. (1) We do not impose coarse-grained synchronization (no need to instrument with advice atomicity) to collect sound traces. (2) We do not block the execution to timestamp events (to process the VCA) which might impose specific schedulings on the execution.
For RQ2, the t-Mon verdict produced by FACTS notifies the user whether the generated trace is suitable for sound monitoring.

#129A.3 + #129C.3.
Section 8.2 shows that most property specification patterns have some causal independence between events. An exciting challenge, which is mentioned in future work, is to leverage this information to reduce the instrumentation of synchronization actions, as discussed in Sec 6.3.

#129B.1 + #129B.2. 
The reported Exec time only reports the program elapsed time (without timestamping) which is the original program + the overhead of the additional instrumented code. The overall overhead is the sum of Exec and VCA (columns 6 and 7 in Table 1).  The t-Mon is also checked asynchronously upon receiving new events from the program. 

#129B.4. 
To force atomicity (as per Section 2), the synchronization block should wrap the program action (e.g. write) and its advice such that they execute atomically. In AspectJ, we can only inject a synchronization block either before or after that write, but we cannot wrap the action since this would require opening a synchronization block in a @before pointcut and closing it in a different @after pointcut. With bytecode instrumentation, this is achievable when the tool allows for inserting bytecode instructions. We implemented this and an example can be found in supplementary material under facts/experiments/fop/inst-fa/MethodCallsFA.java

#129C.1.
As far as we know, monitoring approaches for the detection (not prediction) of behavioral properties in multithreaded programs have always linearized traces without establishing causality. Predictive approaches cleverly construct different partial orders (such as causally-precedes CP, weak-causally-precedes WCP, SHB, ..) that allow them to maximize the exploration of other interleavings. Our purpose is different in that our work attempts to establish causality for the sake of online monitoring. The algorithm can be run asynchronously if needed. Even though our partial order is vanilla HB, it is intended to alarm the monitor/user about incorrect orderings in a linearized trace that are produced during execution by specific scheduling.

#129C.2. 
Maybe we should have included this in an appendix. However, the source code for the tool was provided in the supplementary material. Here are some more details. The bytecode instrumentation logic is given in Java classes. An example can be found under facts/experiments/avrora/inst-facts. We used our instrumentation tool, which is also included in the material. As for the extracted events from the program, it is a tuple of (int name, Long thread, String address, Object resource, Object value). We assumed that event names can be associated with a number which allowed us to optimize many comparison operations. The VCA implementation can be found under facts/src/x/c/facts/vectorclock/algorithm/VectorClockAlgorithm.java. FACTS is implemented in JAVA with 1.5 KLoC. The implementation will be released and made public upon acceptance.

==> tikzold/confused.tex <==
\begin{tikzpicture} [
  node distance=.3cm and .3cm,
  smallarrow/.style={thin, -latex},
  box/.style={circle,draw,minimum width=+3ex,minimum height=+3ex,inner sep=+0pt},
  RA/.style={box, fill=gray!80!black, text=white},
  SA/.style={box, double},
  hidden/.style={ draw=none},
  fit1/.style={dotted, black, rectangle, draw},
  fit2/.style={fit1, solid},
  label/.style={draw = white}]

\lbubble[RA]{t0a0}{}{$x$}
\lbubble[]{t0a1}{right=of t0a0}{$z$}
\lbubble[RA]{t0a2}{right=of t0a1}{$y$}
\lbubble[]{t0a3}{right=of t0a2}{$z$}
\lbubble[RA]{t0a4}{right=of t0a3}{$x$}
\lbubble[RA]{t0a5}{right=of t0a4}{$y$}

\draw[smallarrow] (t0a0) -- (t0a1);
\draw[smallarrow] (t0a1) -- (t0a2);
\draw[smallarrow] (t0a2) -- (t0a3);
\draw[smallarrow] (t0a3) -- (t0a4);
\draw[smallarrow] (t0a4) -- (t0a5);

\lbubble[RA]{t1a0}{right=1.5 of t0a5}{$x$}
\lbubble[RA]{t1a1}{right=of t1a0, yshift=0.5cm, xshift=0.4cm}{$y$}
\lbubble[]{t1a2}{right=of t1a0, yshift=-0.5cm}{$z$}
\lbubble[]{t1a3}{right=of t1a2}{$z$}
\lbubble[RA]{t1a4}{right=of t1a3, yshift=0.5cm}{$x$}
\lbubble[RA]{t1a5}{right=of t1a4}{$y$}


\draw[smallarrow] (t1a0) -- (t1a1);
\draw[smallarrow] (t1a0) -- (t1a2);
\draw[smallarrow] (t1a1) -- (t1a4);
\draw[smallarrow] (t1a2) -- (t1a3);
\draw[smallarrow] (t1a3) -- (t1a4);
\draw[smallarrow] (t1a4) -- (t1a5);

\end{tikzpicture}


==> tikzold/overview.tex <==
\begin{tikzpicture} [
  node distance=.3cm and .3cm,
  smallarrow/.style={thin, -latex},
  box/.style={circle,draw,minimum width=+2ex,minimum height=+2ex,inner sep=+0pt},
  RA/.style={box, fill=gray!80!black},
  SA/.style={box, double},
  hidden/.style={ draw=none},
  fit1/.style={dotted, black, rectangle, draw},
  fit2/.style={fit1, solid},
  label/.style={draw = white}]

% ---------------------------------------------- Classical Approach

\bubble[RA]{t0a0}{xshift=0.7cm}
\bubble[hidden]{t1}{below=of t0a0}
\bubble{t1a0}{right=of t1}

\bubble[]{t0a1}{right=of t0a0}
\bubble[RA]{t0a2}{right=of t0a1}
\bubble{t0a3}{right=of t0a2}
\bubble{t0a4}{right=of t0a3}
\bubble[RA]{t0a5}{right=of t0a4}

\draw[smallarrow] (t0a0) -- (t0a1);
\draw[smallarrow] (t0a1) -- (t0a2);
\draw[smallarrow] (t0a2) -- (t0a3);
\draw[smallarrow] (t0a3) -- (t0a4);
\draw[smallarrow] (t0a4) -- (t0a5);

\bubble[hidden]{t1a1}{right=of t1a0}
\bubble[RA]{t1a2}{right=of t1a1}
\bubble[]{t1a3}{right=of t1a2}

\draw[smallarrow] (t1a0) -- (t1a2);
\draw[smallarrow] (t1a2) -- (t1a3);


\draw[smallarrow] (t0a1) -- (t1a2);
\draw[smallarrow] (t1a3) -- (t0a5);

\node (exec1) [fit2, inner sep=5pt,
                          fit = (t0a0) (t0a5) (t1a3)] {};
\node (labelexec1)[above left] at (exec1.north east) {{\footnotesize Concurrent Execution}};


\node (assum) [fit1, left=0.7 of t0a0, yshift=0.8cm, rotate=90] {\footnotesize Assumptions};


%\node (assum) [fit1, fit = (assum0) (assum2),  inner sep=0pt]{};
\node (inst1) [fit2, inner sep=2pt, fit = (exec1) (labelexec1) (assum)] {};


\node (labelinst1)[above left] at (inst1.north east) {{\footnotesize Instrumentation}};



\bubble[RA]{total-a0}{right=4.1 of t0a1}
\bubble[RA,]{total-a1}{below=of total-a0, xshift=0.3cm}
\bubble[RA]{total-a2}{right=of total-a0}
\bubble[RA,]{total-a3}{right=of total-a2}
\bubble[hidden]{total-fit-fix}{above=0.2 of total-a0}

\draw[smallarrow] (total-a0) -- (total-a1);
\draw[smallarrow] (total-a1) -- (total-a2);
\draw[smallarrow] (total-a2) -- (total-a3);

\node (t-total) [fit2, inner sep=5pt, fit = (total-a0) (total-a1) (total-a3) ]{};
\node (label-t-total)[above] at (t-total.north) {\footnotesize Linear Trace};



\draw[smallarrow] let \p1 = (t-total.west), \p2 = (inst1.east)
    in (\p2) -- (\x1,\y2);

% ---------------------------------------------- Our Approach

\bubble[RA]{1t0a0}{below=2.1  of t0a0, xshift=-0.7cm}
\bubble[hidden]{1t1}{below=of 1t0a0}
\bubble{1t1a0}{right=of 1t1}

\bubble[SA]{1t0a1}{right=of 1t0a0}
\bubble[RA]{1t0a2}{right=of 1t0a1}
\bubble{1t0a3}{right=of 1t0a2}
\bubble{1t0a4}{right=of 1t0a3}
\bubble[SA,RA]{1t0a5}{right=of 1t0a4}

\draw[smallarrow] (1t0a0) -- (1t0a1);
\draw[smallarrow] (1t0a1) -- (1t0a2);
\draw[smallarrow] (1t0a2) -- (1t0a3);
\draw[smallarrow] (1t0a3) -- (1t0a4);
\draw[smallarrow] (1t0a4) -- (1t0a5);

\bubble[hidden]{1t1a1}{right=of 1t1a0}
\bubble[SA,RA]{1t1a2}{right=of 1t1a1}
\bubble[SA]{1t1a3}{right=of 1t1a2}

\draw[smallarrow] (1t1a0) -- (1t1a2);
\draw[smallarrow] (1t1a2) -- (1t1a3);
\draw[smallarrow] (1t0a1) -- (1t1a2);
\draw[smallarrow] (1t1a3) -- (1t0a5);


\node (exec2) [fit2, inner sep=5pt,
                          fit = (1t0a0) (1t0a5) (1t1a3)] {};
\node (labelexec2)[above left] at (exec2.north east) {{\footnotesize Concurrent Execution}};



\node (1assum) [fit2, double, left=1 of 1t0a0, yshift=0.7cm, rotate=90] {\footnotesize Assumptions};
\node (inst2) [fit2, inner sep=3pt, fit = (exec2) (labelexec2)] {};
\node (labelinst2)[above left] at ($(inst2.north east)+(0,-0.05)$) {{\footnotesize Instrumentation}};


\bubble[RA]{partial-a0}{right=5.4 of 1t0a0}
\bubble[RA,SA]{partial-a1}{below=of partial-a0, xshift=0.6cm}
\bubble[RA]{partial-a2}{right=of partial-a0}
\bubble[RA, SA]{partial-a3}{right=of partial-a2}

\draw[smallarrow] (partial-a0) -- (partial-a1);
\draw[smallarrow] (partial-a0) -- (partial-a2);
\draw[smallarrow] (partial-a1) -- (partial-a3);
\draw[smallarrow] (partial-a2) -- (partial-a3);

\node (t-partial) [fit2, inner sep=5pt, fit = (partial-a0) (partial-a1) (partial-a3)]{};
\node (label-t-partial)[above] at (t-partial.north) {\footnotesize Concurrent Trace};



\draw[smallarrow]  let \p1 = ($(inst2.east) + (0, 0.2)$), \p2 = (t-partial.west)
   in (\p1)  -- (\x2,\y1);
\draw[smallarrow]  let \p1 = ($(inst2.west) + (0, -0.1)$), \p2 = (1assum.south)
  in (\x2,\y1) -- (\p1);

%\coordinate (O) at ($ (inst2)!0.7!(t-partial) + (0,-0.1)$);
%\draw[smallarrow,dashed, -]($(t-partial.west) + (0,-0.1)$) -- (O);
%\draw[smallarrow, dashed]  (O) -- ($(1assum.east)$);
%\draw[smallarrow, dashed]  (O) -- ++(0,0.8) -- ($(inst2.east) +(0, 0.7)$);

\draw[smallarrow, dashed,|>-<|] ($(t-partial.west) + (0, -0.45)$) -- ($(exec2.east) + (0, -0.45)$);

\node[label] (lblrel) at ($(t-partial.south west)!0.5!(exec2.south east)+(0.1, 0.4)$) {\scriptsize{sound/faithful?}};

\coordinate (edge1) at ($(inst1.south west)!0.2!(inst2.north west) + (-1.4,0)$);

\draw[smallarrow,-, thin] let \p1 = ($(t-total.south east)!0.4!(t-partial.north east)$), \p2 = (edge1)
  in (edge1) -- (\x1,\y2);

\node[anchor=south west] (lblcur) at ($(edge1) + (0.2,0)$) {\scriptsize{current}};
\node[anchor=north west] (lblprop) at ($(edge1) + (0.1,0)$) {\scriptsize{proposed}};

\end{tikzpicture}


==> tikzold/overview0.tex <==
\begin{tikzpicture} [
  node distance=.3cm and .3cm,
  smallarrow/.style={thin, -latex},
  box/.style={circle,draw,minimum width=+2ex,minimum height=+2ex,inner sep=+0pt},
  RA/.style={box, fill=gray!80!black},
  SA/.style={box, double},
  hidden/.style={ draw=none},
  fit1/.style={dotted, black, rectangle, draw},
  fit2/.style={fit1, solid},
  label/.style={draw = white}]

\bubble[RA]{t0a0}{}
\bubble[hidden]{t1}{right=of t0a0}
\bubble{t1a0}{below=of t1}

\bubble[SA]{t0a1}{below=of t0a0}
\bubble[RA]{t0a2}{below=of t0a1}
\bubble{t0a3}{below=of t0a2}
\bubble{t0a4}{below=of t0a3}
\bubble[SA,RA]{t0a5}{below=of t0a4}

\draw[smallarrow] (t0a0) -- (t0a1);
\draw[smallarrow] (t0a1) -- (t0a2);
\draw[smallarrow] (t0a2) -- (t0a3);
\draw[smallarrow] (t0a3) -- (t0a4);
\draw[smallarrow] (t0a4) -- (t0a5);

\bubble[hidden]{t1a1}{below=of t1a0}
\bubble[SA,RA]{t1a2}{below=of t1a1}
\bubble[SA]{t1a3}{below=of t1a2}

\draw[smallarrow] (t1a0) -- (t1a2);
\draw[smallarrow] (t1a2) -- (t1a3);


\draw[smallarrow] (t0a1) -- (t1a2);
\draw[smallarrow] (t1a3) -- (t0a5);

\node (exec) [fit1, inner sep=10pt,
                          fit = (t0a0) (t0a5) (t1a3)] {};
\node (labelexec)[above left] at (exec.north east) {{\footnotesize C. Execution}};

\node (prog) [fit2, fit = (exec) (labelexec)]{};
\node (labelprog)[above] at (prog.north) {\footnotesize Program};

\node (assum0) [right=0.25 of prog, yshift=-.8cm] {$A_0$};
\node (assum1) [below=0 of assum0] {$A_1$};
\node (assum2) [below=0 of assum1] {$\vdots$};
\node (assum) [fit2, fit = (assum0) (assum2),  inner sep=0.5pt]{};

\node (i0) [below right=0 and 1.2 of prog.north east] {};
\node (i1) [below=4.35 of i0] {};

\node (ins) [fit2, fit = (i0) (i1), inner sep=0.5pt]{};
\node (labelins)[above] at (ins.north) {\footnotesize Instrumentation};


\draw[smallarrow] (prog) -- (ins);
\draw[smallarrow] let \p1 = (ins.west), \p2 = (assum)
    in (assum) -- (\x1, \y2);

\draw[smallarrow] let \p1 = (prog.east), \p2 = (assum)
    in (assum) -- (\x1, \y2);


\bubble[RA]{total-a0}{right=1 of ins, yshift=1.65cm}
\bubble[RA,SA]{total-a1}{right=of total-a0, yshift=-0.3cm}
\bubble[RA]{total-a2}{below=of total-a0}
\bubble[RA,SA]{total-a3}{below=of total-a2}

\draw[smallarrow] (total-a0) -- (total-a1);
\draw[smallarrow] (total-a1) -- (total-a2);
\draw[smallarrow] (total-a2) -- (total-a3);

\node (t-total) [fit1, fit = (total-a0) (total-a1) (total-a3)]{};
\node (label-t-total)[above] at (t-total.north) {\footnotesize Current};

\bubble[RA]{partial-a0}{below=1.4 of total-a2}
\bubble[RA,SA]{partial-a1}{below right=of partial-a0, yshift=-0.1cm}
\bubble[RA]{partial-a2}{below=of partial-a0}
\bubble[RA]{partial-a3}{below=of partial-a2}

\draw[smallarrow] (partial-a0) -- (partial-a1);
\draw[smallarrow] (partial-a0) -- (partial-a2);
\draw[smallarrow] (partial-a1) -- (partial-a3);
\draw[smallarrow] (partial-a2) -- (partial-a3);

\node (t-partial) [fit1, fit = (partial-a0) (partial-a1) (partial-a3)]{};
\node (label-t-partial)[above] at (t-partial.north) {\footnotesize Proposed};

\node (traces) [fit2, fit = (t-partial) (label-t-total), inner sep=3pt]{};
\node (label-traces)[above] at (traces.north) {\footnotesize Trace};

\draw[smallarrow] (ins) -- (traces);

\node (rvin) [right=0.8 of traces] {};
\node (mon) [rectangle, draw, minimum width=+6ex,minimum height=+6ex,inner sep=+0pt,
      right=0.1 of rvin] {Mon};
\node (spec) [above=of mon, anchor=south] {Spec};
\node (ver) [right=of mon] {Verdict};

\node (boxbelow)[below=1.5 of mon]{};
\node (boxabove)[above=1.5 of mon]{};

\draw[smallarrow] (spec) -- (mon);
\draw[smallarrow] (mon) -- (ver);
\node (rv) [fit2, fit = (rvin) (boxbelow) (boxabove) (ver)]{};

\draw[smallarrow] (traces) -- (mon);
\node (label-rv)[above] at (rv.north) {\footnotesize RV};

\end{tikzpicture}


==> tikzold/props/soundfaith.tex <==
\begin{tikzpicture} [
  node distance=.3cm and .3cm,
  smallarrow/.style={thin, -latex},
  box/.style={rectangle,draw,minimum width=+3.8ex,minimum height=+3ex,inner sep=+0pt},
  RA/.style={box, fill=gray!80!black, text=white},
  SA/.style={box, double},
  hidden/.style={ draw=none},
  so/.style={dash dot},
  fit1/.style={dotted, black, rectangle, draw},
  fit2/.style={fit1, solid},
  redundant/.style={},
  label/.style={draw = white}]


\lbubble[SA]{0a0}{}{$\code{l_t}$}
\lbubble[SA]{0a1}{right=of 0a0}{$\code{l_s}$}
\lbubble[RA]{0a2}{right=of 0a1}{$\code{0.w^0}$}
\lbubble[SA]{0a3}{right=of 0a2}{$\code{u_s}$}
\lbubble[SA]{0a4}{right=of 0a3}{$\code{u_t}$}

\lbubble[SA]{0a5}{right=2.1 of 0a4}{$\code{l_t}$}
\lbubble[SA]{0a6}{right=1.2 of 0a5}{$\code{l_s}$}
\lbubble[RA]{0a7}{right=of 0a6}{$\code{1.w^0}$}

\draw[smallarrow] (0a0) -- (0a1);
\draw[smallarrow] (0a1) -- (0a2);
\draw[smallarrow] (0a2) -- (0a3);
\draw[smallarrow] (0a3) -- (0a4);
\draw[smallarrow] (0a4) -- (0a5);
\draw[smallarrow] (0a5) -- (0a6);
\draw[smallarrow] (0a6) -- (0a7);



\lbubble[SA]{1a0}{below=of 0a0}{$\code{l_t}$}
\lbubble[SA]{1a1}{right=of 1a0}{$\code{l_c}$}
\lbubble[]{1a2}{right=of 1a1}{$\code{i}$}
\lbubble[SA]{1a3}{right=of 1a2}{$\code{l_s}$}
\lbubble[SA]{1a4}{right=of 1a3}{$\code{u_c}$}
\lbubble[SA]{1a5}{right=of 1a4}{$\code{u_t}$}
\lbubble[RA]{1a6}{right=of 1a5}{$\code{r^1}$}
\lbubble[SA]{1a7}{right=of 1a6}{$\code{l_c}$}
\lbubble[]{1a8}{right=of 1a7}{$\code{d}$}
\lbubble[SA]{1a9}{right=of 1a8}{$\code{u_s}$}
\lbubble[SA]{1a10}{right=of 1a9}{$\code{u_c}$}

\draw[smallarrow] (1a0) -- (1a1);
\draw[smallarrow] (1a1) -- (1a2);
\draw[smallarrow] (1a2) -- (1a3);
\draw[smallarrow] (1a3) -- (1a4);
\draw[smallarrow] (1a4) -- (1a5);
\draw[smallarrow] (1a5) -- (1a6);
\draw[smallarrow] (1a6) -- (1a7);
\draw[smallarrow] (1a7) -- (1a8);
\draw[smallarrow] (1a8) -- (1a9);
\draw[smallarrow] (1a9) -- (1a10);

\lbubble[SA]{2a0}{below=of 1a0}{$\code{l_t}$}
\lbubble[SA]{2a1}{right=of 2a0}{$\code{l_c}$}
\lbubble[]{2a2}{right=of 2a1}{$\code{i}$}
\lbubble[SA]{2a3}{right=1.2cm of 2a2}{$\code{u_c}$}
\lbubble[SA]{2a4}{right=of 2a3}{$\code{u_t}$}
\lbubble[RA]{2a5}{right=of 2a4}{$\code{r^2}$}
\lbubble[SA]{2a6}{right=of 2a5}{$\code{l_c}$}
\lbubble[]{2a7}{right=of 2a6}{$\code{d}$}
\lbubble[SA]{2a8}{right=of 2a7}{$\code{u_c}$}

\draw[smallarrow] (2a0) -- (2a1);
\draw[smallarrow] (2a1) -- (2a2);
\draw[smallarrow] (2a2) -- (2a3);
\draw[smallarrow] (2a3) -- (2a4);
\draw[smallarrow] (2a4) -- (2a5);
\draw[smallarrow] (2a5) -- (2a6);
\draw[smallarrow] (2a6) -- (2a7);
\draw[smallarrow] (2a7) -- (2a8);

\draw[smallarrow,so] (0a4.south) -- ++(0,-0.1) -- ($(1a0.north) + (0,0.2)$) -- (1a0.north);
\draw[smallarrow,so, redundant] let \p1 = (0a3.south), \p2 = (1a3.north)
  in (0a3.south) -- (\x1, \y2);

\draw[smallarrow,so] (1a5.south) -- ++(0,-0.1) -- ($(2a0.north) + (0,0.2)$) -- (2a0.north);
\draw[smallarrow,so, redundant] (1a4.south) -- ++(0,-0.2) -- ($(2a1.north) + (0,0.1)$) -- (2a1.north);

\draw[smallarrow,so] (2a8.north) -- ++(0,0.1) -- ($(1a7.south) + (0,-0.2)$) -- (1a7.south);
\draw[smallarrow,so] let \p1 =($(2a4.east)+(0,0.1)$), \p2 = ($(0a5.west) + (0,-0.1)$), \p3 = ($(2a4.north)!0.28!(0a5.west)$)
    in  (\p1)  -- ($(\x3, \y1)$) -- (\x3, \y2) -- (\p2);

\draw[smallarrow,so] (1a9) -- (0a6);
%\draw[smallarrow] let \p1 =($(2a4.north)+(0.2,0)$), \p2 = (0a5.west)
%    in  (\p1) -- (\x1, \y2) -- (\p2);

%\lbubble[SA]{t1}{right=of t0w}{$u$}

%\lbubble[]{t0a1}{right=of t0a0}{$z$}
%\lbubble[RA]{t0a2}{right=of t0a1}{$y$}
%\lbubble[]{t0a3}{right=of t0a2}{$z$}
%\lbubble[RA]{t0a4}{right=of t0a3}{$x$}
%\lbubble[RA]{t0a5}{right=of t0a4}{$y$}

%\draw[smallarrow] (t0a0) -- (t0a1);



\end{tikzpicture}


==> title.tex <==
\title{Runtime Verification of Multithreaded Programs}
%
%
\author{
  Chukri~Soueidi,  Yli\`{e}s~Falcone\\
  % Univ.~Grenoble~Alpes,~Inria,\\ 
  % CNRS,~Grenoble~INP,~LIG\\ 
  % 38000~Grenoble\\ 
  % France \\
  % \texttt{chukri.a.soueidi@inria.fr} \\
  %
  % \And
  % Ali~Kassem\\
  % Univ.~Grenoble~Alpes,~Inria,\\ 
  % CNRS,~Grenoble~INP,~LIG\\ 
  % 38000~Grenoble\\ 
  % France \\
  % \texttt{ali.kassem@inria.fr} \\
  % %
  % \And
  % Yli\`{e}s~Falcone\\
  % Univ.~Grenoble~Alpes,~Inria,\\ 
  % CNRS,~Grenoble~INP,~LIG\\ 
  % 38000~Grenoble\\ 
  % France \\
  % \texttt{ylies.falcone@inria.fr} \\
}



